2D-DPO: Scaling Direct Preference Optimization with 2-Dimensional Supervision

Recent advancements in Direct Preference Optimization (DPO) have significantly enhanced the alignment of Large Language Models (LLMs) with human preferences, owing to its simplicity and effectiveness. However, existing methods typically optimize a scalar score or ranking reward, thereby overlooking the multi-dimensional nature of human preferences. In this work, we propose to extend the preference of DPO to two dimensions: segments and aspects. We first introduce a 2D supervision dataset called HelpSteer-2D. For the segment dimension, we divide the response into sentences and assign scores to each segment. For the aspect dimension, we meticulously design several criteria covering the response quality rubrics. With the 2-dimensional signals as feedback, we develop a 2D-DPO framework, decomposing the overall objective into multi-segment and multi-aspect objectives. Extensive experiments on popular benchmarks demonstrate that 2D-DPO performs better than methods that optimize for scalar or 1-dimensional preferences.

==> content/1_introduction_20241014.tex <==
\section{Introduction}

Recent advancements in large language models (LLMs), such as GPT-4 and LLaMA~\cite{openai2023gpt,touvron2023llama}, have demonstrated remarkable performance across various text generation tasks~\cite{zhao2023survey}. A pivotal component in LLM training is Reinforcement Learning from Human Feedback (RLHF) ~\cite{ouyang2022training, bai2022training}, which aligns LLM with human values and intentions. 
% RLHF typically involves the development of a reward model followed by the fine-tuning of the policy model using reinforcement learning. The reward model learns to determine desirable behaviour based on human feedback, which is used to guide the policy to determine the agent's actions~\cite{stiennon2020learning}.
However, due to its complexity, traditional RLHF often presents challenges such as training instability and reward collapse ~\cite{wolf2023fundamental, song2023reward}. As an alternative, Direct Preference Optimization (DPO)~\cite{rafailov2023direct} has gained significant traction attributed to its simplicity and effectiveness. DPO directly adjusts the model parameters based on preference data, bypassing the explicit fitting of a reward model. Numerous variations of DPO have been proposed, extending the method to reference-free~\cite{meng2024simpo} or binary feedback scenarios~\cite{ethayarajh2024kto}.

Despite the progress that has been made, existing works mostly ignore the intricacy of human preferences, which inherently comprise different dimensions.
On one hand, a response may be deemed satisfactory under one aspect but may fall short under another. On the other hand, not all segments are to be approved or punished for a single response. Existing methods rely on a singular reward to optimize the model output~\cite{rafailov2023direct, meng2024simpo}, resulting in inefficient or inaccurate supervision. Therefore, many researchers begin to explore how to obtain fine-grained signals and incorporate them into training. Some work leverage signals that are believed to be related to the importance of segments as reward scores~\cite{zeng2024token, chan2024dense, jiang2024bridging, chen2024improving}.
% However, these signals are based on statistical features such as edit distance or confidence estimation, which can introduce additional noise and lead to training instability. 
Other work incorporates multi-objective optimization and aims to strike a balance between different aspects of human preferences~\cite{wu2024fine, guo2023beyond, cao2024drlc}. 
% However, these methods are typically conducted on reinforcement learning approaches such as Proximal Policy Optimization (PPO), which cannot be directly combined with direct preference alignment.
However, all of these efforts only scale preference optimization from 0-dimension (scalar reward) to 1-dimension (aspect/segment), which is insufficient to align with real-world human preferences.

% On the other hand, chosen and rejected answers may have similar content, but in actual training, opposite optimization goals are accepted, which will lead to training conflicts or uncontrollable. 

% Despite several attempts to incorporate token-level feedback into the training process~\cite{lightman2023let, wu2024fine, zeng2024token, yang2024preference, wang2024math}, there still exist some limitations.
%In acquiring fine-grained signals, the fine-grained signals of most methods are still singular or lack basis. For example, some methods can only provide one or two types of feedback without considering the different degrees of preference of each token, such as FIGA~\cite{guo2023beyond} and DRLC~\cite{cao2024drlc}. Some methods leverage other signals that are believed to be related to the importance of tokens as reward scores, such as confidence and attention scores. Examples of such methods include TRLC~\cite{zeng2024token}, ABC~\cite{chan2024dense}, and BMC~\cite{jiang2024bridging}. However, the research community still doubts their interpretability~\cite{jain2019attention, serrano2019attention, bibal2022attention}, which can easily introduce additional noise and lead to instability during training. 
%In fine-grained alignment training strategy, many of these methods only apply to traditional reinforcement learning approaches such as Proximal Policy Optimization(PPO)~\cite{ouyang2022training, wu2024fine, guo2023beyond, cao2024drlc, chen2024improving, chan2024dense} that cannot be directly combined with direct preference alignment methods.

% FGMO这个名字感觉得换一个
To better counter with the intricacy of human preferences, we propose 2D-DPO, a novel direct alignment strategy that enables 2-dimensional (2D) fine-grained optimization. 
% 介绍核心思想
Our core idea is to scale the supervision signals to segment-dimension and aspect-dimension. Each sample is annotated with a 2-dimensional score matrix assigned for each segment and each aspect. The signals are derived from a strong model guided by a set of strict principles, which ensure the production of highly accurate and detailed signals. After that, we utilize a novel strategy to achieve 2-dimensional direct preference alignment. Compared with previous methods, our method not only reflects the degree for each segment but also reflects the aspect of that preference. Additionally, our method offers more accurate and fair reward guidance by extracting a set of principles to formulate quantifiable standards in natural language strictly. 
%Moreover, our method extends DPO to two-dimensional fine-grained optimization at minimal cost, ensuring stability and achieving high computational efficiency.

% To ensure the reproducibility of our work, we construct a preference dataset called xxx containing two-dimensional (2D) fine-grained signals (token-level and multi-objective). We also trained a reward model that can annotate the two-dimensional fine-grained signal based on this annotated seed data, which has a high consistency rate with human annotations. 
% Compared with previous methods, our method can provide more fine-grained token-level guidance. Specifically, it not only captures the preference for each token but also reflects the degree and type of that preference. Additionally, our method offers more accurate and fair reward guidance by drawing on the practice of constitutional AI to formulate quantifiable standards in natural language strictly.
% The last key point is that our method is an RL-free algorithm that extends DPO to two-dimensional fine-grained optimization at minimal cost, ensuring stability and achieving high computational efficiency.

We construct a preference dataset named HelpSteer-2D with 2-dimensional fine-grained reward signals \cite{wang2024helpsteer2}. Based on the dataset, we compare different preference optimization methods on Llama3-8B and Qwen-2-7B \cite{llama3modelcard, qwen2}. Experiment results on instruction-following benchmarks demonstrate that 2D-DPO surpasses previous methods by a large margin. We also trained a 2D-reward model to provide an online reward signal upon both token-level and aspect-level, which presents high consistency with human annotations.

==> content/2_RelatedWork_20241014.tex <==

\section{Related Work}
\subsection{Preference Optimization}

Large language models (LLMs) have advanced rapidly, with reinforcement learning from human feedback (RLHF) commonly used to align LLMs with human preferences~\citep{ziegler2019fine, stiennon2020learning, ouyang2022training, bai2022training, zhao2023survey}. However, traditional RLHF methods face challenges like instability and high resource demands~\cite{wolf2023fundamental, song2023reward}, prompting the search for simpler alternatives. 
One such representative approach is Direct Preference Optimization (DPO)~\cite{rafailov2023direct}, which optimizes alignment without explicit reward modeling, offering simplicity and stability. Building on DPO, IPO~\cite{azar2024general} adds a regularization term to alleviate overfitting. KTO~\cite{ethayarajh2024kto} only requires a binary signal of whether an output is desirable or undesirable for an input to align LLMs, simplifying the data acquisition process. ORPO~\cite{hong2024reference} simplifies training with odds ratio-based penalties, and SimPO~\cite{meng2024simpo} improves efficiency by using average log probability as an implicit reward.

\subsection{Token-level Preference Optimization}

The response-level reward for the model's output makes it difficult to capture the details of specific tokens in the sequence, leading to inefficient and unstable learning. Therefore, many researchers began to explore how to obtain fine-grained signals and introduce such fine-grained supervision signals into training.

Existing methods for obtaining fine-grained signals are mainly divided into three categories. The first category involves human annotation, as explored by ~\citeauthor{lightman2023let} and ~\citeauthor{wu2024fine}, where human annotators label each segment of the model’s output. The second category leverages stronger LLMs to obtain fine-grained signals, which can be further divided into two subcategories: (1) utilizing external LLM to generate preference pairs with minimal edits, offering specific token-level guidance by comparing modified parts~\cite{guo2023beyond,chen2024improving,yoon2024tlcr,jiang2024bridging}; (2) directly employing external LLMs to identify the positive and negative parts of the generated response, as seen in methods like DRLC~\citep{cao2024drlc}. The third category employs the endogenous information of the model as a reward signal, such as ABC~\cite{chan2024dense} using attention scores as token reward scores and SePO~\cite{yang2024selective} leverages the insight that DPO inherently learns a reward function that decomposes response-level reward values into token-level rewards~\cite{rafailov2024r} to produce token selection signals. For fine-grained training strategies, most methods use traditional RL algorithms such as PPO~\cite{schulman2017proximal}. In addition, TDPO~\cite{zeng2024token} achieves token-level alignment by controlling the KL divergence for each token.
Despite these advancements, several limitations persist. Some can only provide binary feedback, failing to consider the different degrees of preference for each token(such as RELC). Some use indirect signals as reward scores like confidence and attention scores, which can easily introduce additional noise signals and lead to training instability(such as TRLC, ABC, and BMC). At the same time, most methods only apply to traditional RL methods, such as PPO, and cannot be directly combined with direct preference alignment methods. 

%Additionally, several studies also explore token-level preference optimization to enhance models’ mathematical reasoning abilities~\cite{lightman2023let,wang2024math,ma2023let,xie2024monte,lai2024step}. However, these approaches are often limited to specific domains like mathematics, where answers are definitive and step-by-step reasoning is required. Our study, by contrast, focuses on more general natural language scenarios.

% 这里还不确定要不要单独说多目标...
\subsection{Multi-objective Preference Optimization}

Humans often exhibit complex, diverse, or even contradictory preferences, which complicates training a model based on single-dimensional supervised preference information. To address this, some studies explore aligning LLMs with multiple alignment objectives. A common approach is to directly train a separate reward model for each objective and then convert the multi-objective reward to a scalar using the weights of each objective~\cite{pan2023rewards,ji2024beavertails,rame2024rewarded,de2024reinforcement}. Alternatively, a linear combination of the multi-dimensional objectives can be directly fitted during training~\cite{wang2024arithmetic}. However, this approach demands significant computational resources. In contrast, \citeauthor{zhou2024beyond} proposes a reinforcement learning-free algorithm that extends direct preference optimization for multiple alignment objectives while minimizing overhead. Furthermore, other strategies employ customized hinting techniques to integrate multiple reward values, optimized through supervised fine-tuning, to enhance controllable generation during inference \cite{yang2024rewards, guo2024controllable}.
